Nonuniqueness and existence of continuous, globally dissipative Euler flows

We show that H\"{o}lder continuous incompressible Euler flows that satisfy the local energy inequality ("globally dissipative" solutions) exhibit nonuniqueness and contain examples that strictly dissipate kinetic energy. The collection of such solutions emanating from a fixed initial data may have positive Hausdorff dimension in the energy space even if the local energy equality is imposed, and the set of initial data giving rise to such an infinite family of solutions is $C^0$ dense in the space of continuous, divergence free vector fields on the torus ${\mathbb T}^3$. The construction of these solutions involves a new and explicit convex integration approach mirroring Kraichnan's LDIA theory of turbulent energy cascades that overcomes the limitations of previous schemes, which had been restricted to bounded measurable solutions or to continuous solutions that dissipate total kinetic energy.

==> betterBoundStress.tex <==
Recall from \eqref{eq:stressDecomp} that the new stress $\ost{R}^{j\ell} = R_T^{j\ell} + R_S^{j\ell} + R_H^{j\ell} + R_M^{j\ell}$ will be decomposed into four terms.  The terms $R_T^{j\ell}$ and $R_H^{j\ell}$ are symmetric tensors that must solve the equations.%, called the {\bf symmetric divergence equation}
\ali{
\nb_j R_T^{j\ell} &= \pr_t V^\ell + \nb_j[v_\ep^j V^\ell + V^j v_\ep^\ell] \notag \\
&= \pr_t V^\ell + v_\ep^j  \nb_j V^\ell + V^j  \nb_j v_\ep^\ell \label{eq:transportTermThird} \\
\nb_j R_H^{j\ell} &= \sum_{J \neq \bar{I}} \nb_j( V_I^j V_J^\ell) \label{eq:highFreqTermThird}
}
Observe that right hand sides of \eqref{eq:transportTermThird} and \eqref{eq:highFreqTermThird} both have frequency support contained in the annulus 
\ali{
\Fsupp \eqref{eq:transportTermThird} \cup \Fsupp \eqref{eq:highFreqTermThird} \subseteq \{ B_\la \osn \Xi \leq |m|  \lsm B_\la \osn \Xi \} \subseteq \widehat{\R^3}. \label{eq:containFreq}
}
This containment follows from the fact that the Fourier transform maps products to convolutions, the containment $\Fsupp V_I \subseteq \{ 2 B_\la \osn \Xi \leq (n_I/3) B_\la \osn \Xi \leq |m| \leq 3 n_I B_\la \osn \Xi \}$ for $n_I$ chosen appropriately in Section~\ref{sec:constrShape}, and the containment $\Fsupp v_\ep \subseteq \{ |m| \leq (1/10) \osn^{1/2} \Xi \}$ for $c_0$ chosen small in \eqref{eq:vMinusVepbd}.

Now let $Q_a^{j\ell} \ast$ be an order $-1$, right-inverse for the divergence operator taking values in symmetric tensors and let $Q_{a, \approx \la}^{j\ell}  \ast = P_{\approx \la} Q_a^{j\ell} \ast$ be the same operator but localized to frequencies of order $\la$ by a Fourier multiplier $P_{\approx \la} = \chi_{\approx \la} \ast$ whose symbol is a smooth, rescaled cutoff function $\widehat{\chi_{\approx \la}}(m) = \widehat{\chi_{\approx 1}}(m/\la)$ supported in $\Fsupp \chi \subseteq \{ \la/2 \leq |m| \lsm \la \}$ with $\hat{\chi}_{\approx \la}(m) = 1$ on \eqref{eq:containFreq}.  We solve \eqref{eq:transportTermThird}-\eqref{eq:highFreqTermThird} by setting
\ali{
R_T^{j\ell} &= Q_{a, \approx \la}^{j\ell} \ast [ \Ddt V^a + V^b \nb_b v_\ep^a  ], \qquad 
R_H^{j\ell} = \sum_{J \neq \bar{I}} Q_{a, \approx \la}^{j\ell} \ast [ \nb_j( V_I^j V_J^\ell)   ]. \label{eq:defOfRTRH}
}
One example of an order $-1$ inverse to the divergence is the Fourier-multiplier whose symbol is
\ali{
\begin{split}
\widehat{Q}_{a}^{j\ell}(m) &= (-i) \left( \widehat{Q}_{a \parallel}^{j\ell}(m) + \widehat{Q}_{a\perp}^{j\ell}(m) \right) \\
\widehat{Q}_{a \parallel}^{j\ell}(m) &= |m|^{-2} m_a \de^{j\ell}, \quad \widehat{Q}_{a\perp}^{j\ell}(m) = |m|^{-2}(m^j \de_a^\ell + \de_a^j m^\ell) - 2 |m|^{-4}(m^j m^\ell m_a ).
\end{split}
}
The properties we need are that $\widehat{Q}_{a}^{j\ell}(m)$ is symmetric in $j\ell$, degree $-1$ homogeneous, smooth away from $0$, and satisfies $i m_j \widehat{Q}_a^{j\ell}(m) = m^\ell$.  With these properties, we have that $Q_{a,\approx \la}^{j\ell}(h)$ %= \la^{-1} ( \la^3 Q_{a, \approx 1}^{j\ell}(\la h) )$ 
is a rescaling of a Schwartz function with $\widehat{Q}_{a,\approx \la}^{j\ell}(m) = \la^{-1} \widehat{\chi_{\approx 1}}(m/\la) \widehat{Q}_a^{j\ell}(m/\la)$, and that $R_T^{j\ell}$ and $R_H^{j\ell}$ defined in \eqref{eq:defOfRTRH} solve \eqref{eq:transportTermThird}-\eqref{eq:highFreqTermThird} and satisfy the containment \eqref{eq:containFreq}.  In physical space, the kernel takes the form $Q_{a,\approx \la}^{j\ell}(h) = \la^{-1} ( \la^3 Q_{a, \approx 1}^{j\ell}(\la h) ) $ with $Q_{a, \approx 1}^{j\ell}$ a fixed Schwartz function.  Consequently, $Q_{a,\approx \la}^{j\ell}(h)$ satisfies the hypotheses of Lemma~\ref{lem:commutator} with $\La^{-1} \lsm \la^{-1}$.  Applying Lemma~\ref{lem:commutator} to \eqref{eq:defOfRTRH} and using the estimates
\ali{
\co{ \Ddt V^a + V^b \nb_b v_\ep^a } &\lsm \ostu^{-1} e_\vp^{1/2}  + e_\vp^{1/2} \Xi e_v^{1/2} \\ 
\co{\Ddt ( \Ddt V^a + V^b \nb_b v_\ep^a )} &\lsm \ostu^{-1} (\ostu^{-1} e_\vp^{1/2}  + e_\vp^{1/2} \Xi e_v^{1/2}  ),
}
which follows from \eqref{eq:velocBd3} and \eqref{eq:highFreqCorrect}, we obtain the estimate $\brh[R_T] \lsm \la^{-1} \ostu^{-1} e_\vp^{1/2}$.

Turning now to $R_H^{j\ell}$, we calculate
\ali{
 \nb_j( V_I^j V_J^\ell) = V_I^j \nb_j V_J^\ell &= \VR_I^j \nb_j \VR_J^\ell + \de V_I^j \nb_j V_J^\ell + \VR_I^j \de V_J^\ell \\
\VR_I^j \nb_j \VR_J^\ell &= (i \la) e^{i \la (\xi_I + \xi_J)} v_I^j \nb_j \xi_J v_I^\ell = (i \la) e^{i \la (\xi_I + \xi_J)} ( \hat{\de} v_I^j \nb_j \hxii_J + v_I^j \hat{\de} \nb_j \xi_J ) v_I^\ell,
}
where we have used $v_I^j = \hat{v}_I^j + \hat{\de} v_I^j$, $\nb \xi_J = \nb \hxii_J + \hat{\de} \nb \xi_J$ and $\hat{v}_I^j \nb_j \hxii_J = 0$. 
